Group-based Fair Learning Leads to Counter-intuitive Predictions

A number of machine learning (ML) methods have been proposed recently to maximize model predictive accuracy while enforcing notions of group parity or fairness across sub-populations. We propose a desirable property for these procedures, slack-consistency: For any individual, the predictions of the model should be monotonic with respect to allowed slack (i.e., maximum allowed group-parity violation). Such monotonicity can be useful for individuals to understand the impact of enforcing fairness on their predictions. Surprisingly, we find that standard ML methods for enforcing fairness violate this basic property. Moreover, this undesirable behavior arises in situations agnostic to the complexity of the underlying model or approximate optimizations, suggesting that the simple act of incorporating a constraint can lead to drastically unintended behavior in ML. We present a simple theoretical method for enforcing slack-consistency, while encouraging further discussions on the unintended behaviors potentially induced when enforcing group-based parity.

==> exp.tex <==
\section{Experiments}




\begin{table*}
\setlength{\tabcolsep}{2pt}
\begin{center}
  \caption{{\bf Experiment Results: Benchmark Fairness Tasks}: Each row corresponds to a dataset and fairness notion.  We show the accuracy and fairness violation of training with no constraints (Unc.), with  post-processing calibration (Cal.), the Lagrangian approach (Lagr.) and our method. {\bf Bolded} is the method achieving lowest fairness violation for each row. All reported numbers are evaluated on the test set.}
  \label{tab:experiments}
  \begin{tabular}{|l|l|rr|rr|rr|rr|}
 \hline
 & Metric & Unc. Err. & Unc. Vio. & Cal. Err. & Cal. Vio. & Lagr. Err. & Lagr. Vio. & Our Err. &  Our Vio. \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{Bank}} & Dem. Par. & 9.41\%  & .0349 & 9.70\% & .0068 & 10.46\% & .0126 &  9.63\% & {\bf  .0056} \\
 & Eq. Opp. & 9.41\%  & .1452 & 9.55\% & .0506 & 9.86\% & .1237 &  9.48\% & {\bf .0431} \\
 & Eq. Odds & 9.41\%  & .1452 & N/A & N/A  & 9.61\% & .0879 &  9.50\% & {\bf .0376} \\
 & Disp. Imp. & 9.41\%  & .0304 & N/A & N/A  & 10.44\% & .0135 &  9.89\% & {\bf .0063} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{COMPAS}}  & Dem. Par. & 31.49\%  & .2045 & 32.53\% & .0201 & 40.16\% & .0495 & 35.44\% & {\bf .0155} \\
  &Eq. Opp. & 31.49\%  & .2373 & 31.63\% & {\bf .0256} & 36.92\% & .1141 & 33.63\% & .0774 \\
  & Eq. Odds & 31.49\%  & .2373 &  N/A & N/A  & 42.69\% & {\bf .0566} & 35.06\% & .0663 \\
  & Disp. Imp. & 31.21\%  & .1362 &  N/A & N/A  & 40.35\% & .0499 & 42.64\% & {\bf .0256} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{Comm.}} & Dem. Par.& 11.62\% & .4211 & 32.06\%  & .0653 &   28.46\% & .0519 & 30.06\% & {\bf .0107} \\
  & Eq. Opp.& 11.62\% & .5513 & 17.64\%  & {\bf .0584} & 28.45\% & .0897 & 26.85\% & .0833 \\
  & Eq. Odds & 11.62\% & .5513 &  N/A & N/A  & 28.46\% & .0962 & 26.65\% & {\bf .0769} \\
  & Disp. Imp.& 14.83\% & .3960 &  N/A & N/A  & 28.26\% & .0557 & 30.26\% & {\bf .0073} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{German}}  & Dem. Par. & 24.85\% & .0766 & 24.85\%& .0346 & 25.45\%  &  .0410 & 25.15\% &  {\bf .0137} \\
  &Eq. Opp. & 24.85\% & .1120 & 24.54\% & .0922 & 27.27\%  &  .0757 & 25.45\% &  {\bf .0662} \\
  & Eq. Odds & 24.85\% & .1120 &  N/A & N/A  & 34.24\%  &  .1318 & 25.45\% & {\bf .1099} \\
  & Disp. Imp. & 24.85\% & .0608 &  N/A & N/A  & 27.57\%  &  .0468 & 25.15\% &  {\bf .0156}\\
  \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{Adult}}  & Dem. Par. & 14.15\% & .1173 & 16.60\% & .0129 & 20.47\% & .0198 & 16.51\% & {\bf .0037} \\
  & Eq. Opp. & 14.15\% & .1195 & 14.43\% & .0170 & 19.67\% & .0374 & 14.46\% & {\bf .0092} \\
  & Eq. Odds & 14.15\% & .1195 &  N/A & N/A & 19.04\% & {\bf .0160} & 14.58\% & .0221 \\
  & Disp. Imp. & 14.19\% & .1108 &  N/A & N/A & 20.48\% & {\bf .0199} & 17.37\% & .0334 \\
\hline
\end{tabular}
\end{center}
\end{table*}


Our main results are presented in Table~\ref{tab:experiments}.  We compare our method for learning fair classifiers on a number of benchmark datasets: Bank Marketing~\cite{lichman2013uci}, Communities and Crime \cite{lichman2013uci}, ProPublica’s COMPAS \cite{propublica2018}, German Statlog Credit Data \cite{lichman2013uci}, and Adult \cite{lichman2013uci}.
We compare results at satisfying various fairness constraints between our method and the post-processing calibration method (note this method is not applicable to disparate impact) and the Lagrangian method based on~\cite{eban2017scalable}.  See the Appendix for additional details.

We see that our method consistently leads to more fair classifiers, often yielding a classifier with the lowest test violation out of all methods.  
We also include test error rates in the results.  Although the primary objective of these algorithms is to yield a fair classifier, we find that our method is able to find reasonable trade-offs between fairness and accuracy. Our method often provides either better or comparative predictive error than the other fair classification methods (see Figure~\ref{fig:charts_full} for more insight into the trade-offs found by our algorithm).

The results in Table~\ref{tab:experiments} also highlight the disadvantages of existing methods for training fair classifiers.  Although the calibration method is an improvement over an unconstrained model, it is often unable to find a classifier with lowest bias.  %This aligns with previous work~\cite{woodworth2017learning}, which showed that despite the fact that post-processing calibration strives to achieve fairness without regards to accuracy, there exist certain cases where post-processing is provably suboptimal.

We also find the results of the Lagrangian approach to not consistently provide fair classifiers.  
As noted in previous work~\cite{cotter2018optimization,goh2016satisfying}, constrained optimization can be inherently unstable or requires a certain amount of slack in the objective as the constraints are typically relaxed to make gradient-based training possible and for feasibility purposes. Moreover, due to the added complexity of this method, it can overfit and have poor fairness generalization as noted in~\cite{cotter2018training}. 
Accordingly, we find that the Lagrangian method often yields poor trade-offs in fairness and accuracy, at times yielding classifiers with both worse accuracy and more bias. 

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.4\textwidth]{figures/Adult}
    \vspace{-0.2in}
    \end{center}
  \caption{{\bf Results as $\lambda$ changes}: We show test error and fairness violations for demographic parity on Adult as the weightings change. We take the optimal $\lambda = \lambda^*$ found by Algorithm~\ref{alg:demparity}. Then for each value $x$ on the $x$-axis, we train a classifier with data weights based on the setting $\lambda = x\cdot \lambda^*$ and plot the error and violations. We see that indeed, when $x = 1$, we train based on the $\lambda$ found by Algorithm~\ref{alg:demparity} and thus get the lowest fairness violation. On the other hand, $x=0$ corresponds to training on the unweighted dataset and gives us the lowest prediction error. Analogous charts for the rest of the datasets can be found in the Appendix. }
	\label{fig:charts_full}
\end{figure}


==> intro.tex <==
\section{Introduction}

Machine learning has become widely adopted in a variety of real-world applications that significantly affect people's lives~\cite{tsa,loans}. Fairness in these algorithmic decision-making systems has thus become an increasingly important concern: It has been shown that without appropriate intervention during training or evaluation, models can be biased against certain groups~\cite{angwin,hardt2016equality}. 
This is due to the fact that the data used to train these models often contains biases that become reinforced into the model~\cite{bolukbasi2016man}. Moreover, it has been shown that simple remedies, such as ignoring the features corresponding to the protected groups, are largely
ineffective due to redundant encodings in the data \cite{pedreshi2008discrimination}.
In other words, the data can be inherently biased in possibly complex ways, thus making it difficult to achieve fairness.

Research on training fair classifiers has therefore received a great deal of attention. 
One such approach has focused on developing {\em post-processing} steps to enforce fairness on a learned model~\cite{doherty2012information,feldman2015computational,hardt2016equality}.  That is, one first trains a machine learning model, resulting in an unfair classifier.  The outputs of the classifier are then calibrated to enforce fairness.
Although this approach is likely to decrease the bias of the classifier, by decoupling the training from the fairness enforcement, this procedure may not lead to the best trade-off between fairness and accuracy.
Accordingly, recent work has proposed to incorporate fairness into the training algorithm itself, framing the problem as a constrained optimization problem and subsequently applying the method of {\em Lagrange multipliers} to transform the constraints to penalties~\cite{zafar2015fairness,goh2016satisfying,cotter2018two,agarwal2018reductions}; however such approaches may introduce undesired complexity and lead to more difficult or unstable training~\cite{cotter2018two,cotter2018optimization}.
Both of these existing methods address the problem of bias by adjusting the machine learning model rather than the data, despite the fact that oftentimes it is the training data itself -- i.e., the observed features and corresponding labels -- which are biased.
%Popular approaches include {\it post-processing}~\cite{doherty2012information,feldman2015computational,hardt2016equality}, which involves calibrating the outputs of the classifier depending on group attributes, and {\it constrained optimization}~\cite{zafar2015fairness,goh2016satisfying,cotter2018two,agarwal2018reductions}, which uses penalties added to the training loss to encourage fairness. Neither the constrained optimization perspective nor the post-processing method address the root of the problem: The data itself -- i.e., the observed features and corresponding labels themselves -- are biased.


%We focus on methods for training classifiers to satisfy various notions of fairness such as demographic parity, equalized odds, and disparate impact.

%One approach has focused on developing {\em post-processing} steps to enforce fairness on a learned model~\cite{doherty2012information,feldman2015computational,hardt2016equality}.  That is, one first trains a machine learning model, resulting in an unfair classifier.  The outputs of the classifier are then calibrated to enforce fairness.
%Although this approach is guaranteed to achieve fairness, by decoupling the training from the fairness enforcement, this procedure may not lead to the best trade-off between fairness and accuracy.
%Accordingly, recent work has proposed to incorporate fairness into the training algorithm itself, framing the problem as a constrained optimization problem and subsequently applying the method of {\em Lagrange multipliers} to transform the constraints to penalties~\cite{zafar2015fairness,goh2016satisfying,cotter2018two,agarwal2018reductions}. %; however such approaches may introduce undesired complexity and lead to more difficult or unstable training.
%Current approaches to constrained optimization require many hyperparameters and the use of complicated or unstable training procedures~\cite{cotter2018two,cotter2018optimization}.
%Neither the constrained optimization perspective nor the post-processing method address the root of the problem: The data itself -- i.e., the observed features and corresponding labels themselves -- are biased.
%Both of these methods address the problem of bias by adjusting the machine learning model rather than the data, despite the fact that oftentimes it is the data itself -- i.e., the observed features and corresponding labels -- which are biased. %As such, neither post-processing nor the Lagrangian approach may be the most natural or straightforward approach to fair classification.   

\begin{figure*}[t]
\centering
\includegraphics[width=0.98\columnwidth]{diagram.pdf}
\caption{In our approach to training an unbiased, fair classifier, we assume the existence of a true but unknown label function which has been adjusted by a biased process to produce the labels observed in the training data.  Our main contribution is providing a procedure that appropriately weights examples in the dataset, and then showing that training on the resulting loss corresponds to training on the original, true, unbiased labels.}
\label{fig:design}
\end{figure*}

In this paper, we provide an approach to machine learning fairness that addresses the underlying data bias problem directly.
We introduce a new mathematical framework for fairness in which we assume that there exists an {\it unknown} but {\it unbiased} ground truth label function and that the labels observed in the data are assigned by an agent who is possibly biased, but otherwise has the intention of being accurate. 
This assumption is natural in practice, where the observed data may be the result of manual labelling done by actors (e.g. human decision-makers) who strive to provide an accurate label while being affected by (potentially unconscious) biases; or in cases where the observed labels correspond to a process (e.g. results of a written exam) devised to be accurate and fair, but which is nevertheless affected by inherent biases.
%This assumption is natural in practice and may also be applied to settings where the features themselves are biased and that the observed labels were generated by a process depending on the features (i.e. situations where there is bias in both the features and labels). 

Based on this mathematical formulation, we show how one may identify the amount of bias in the training data as a closed form expression.  Furthermore, our derived form for the bias suggests that its correction may be performed by assigning appropriate weights to each example in the training data. We show, with theoretical guarantees, that training the classifier under the resulting weighted objective leads to an unbiased classifier on the original un-weighted dataset. Notably, many pre-processing approaches and even constrained optimization approaches (e.g. \cite{agarwal2018reductions}) optimize a loss which possibly modifies the observed labels or features, and doing so may be legally prohibited as it can be interpreted as training on {\it falsified} data; see~\cite{barocas2016big} (more details about this can be found in Section~\ref{section:related_work}). In contrast, our method {\em does not} 
modify any of the observed labels or features. Rather, we correct for the bias by changing the distribution of the sample points via re-weighting the dataset.

%Notably, the recent constrained optimization approach of \cite{agarwal2018reductions} to fair classification also leads to minimizing a re-weighted loss. However, in their case, depending on the fairness constraint and the Lagrange multipliers learned, the labels used in the re-weighted loss may not be the same as the original observed labels, thus penalizing the model for predicting correctly. While this may be a reasonable approach, training on {\it modified} labels may be legally prohibited \cite{barocas2016big}. Our framework leads to a re-weighted loss without any modifications of the data. 

Our resulting method is general and can be applied to various notions of fairness, including demographic parity, equal opportunity, equalized odds, and  disparate impact. Moreover, the method is practical and simple to tune: With the appropriate example weights, any off-the-shelf classification procedure can be used on the weighted dataset to learn a fair classifier. Experimentally, we show that on standard fairness benchmark datasets and under a variety of fairness notions our method can outperform previous approaches to fair classification.   

==> related.tex <==
\section{Related Work}\label{section:related_work}

Work in fair classification can be categorized into three approaches: post-processing of the outputs, the Lagrangian approach of transforming constraints to penalties, and pre-processing training data. 

{\bf Post-processing}: One approach to fairness is to perform a post-processing of the classifier outputs. Examples of previous work in this direction include \cite{doherty2012information,feldman2015computational,hardt2016equality}. However, this approach of calibrating the outputs to encourage fairness has limited flexibility. \cite{pleiss2017fairness} showed that a deterministic solution is only compatible with a single error constraint and thus cannot be applied to fairness notions such as equalized odds. Moreover, decoupling the training and calibration can lead to models with poor accuracy trade-off. In fact  \cite{woodworth2017learning} showed that in certain cases, post-processing can be provably suboptimal. Other works discussing the incompatibility of fairness notions include \cite{chouldechova2017fair,kleinberg2016inherent}. 

{\bf Lagrangian Approach}: There has been much recent work done on enforcing fairness by transforming the constrained optimization problem via the method of Lagrange multipliers. Some works \cite{zafar2015fairness,goh2016satisfying} apply this to the convex setting.
In the non-convex case, there is work which frames the constrained optimization problem as a two-player game~\cite{kearns2017preventing,agarwal2018reductions,cotter2018two} .
%The resulting classifier in this case is
%a randomized distribution over classifiers.
Related approaches include \cite{edwards2015censoring,corbett2017algorithmic,narasimhan2018learning}.
There is also recent work similar in spirit which encourages fairness by adding penalties to the objective; e.g, \cite{donini2018empirical} studies this for kernel methods and \cite{komiyama2018nonconvex} for linear models.
%However, there are a number of underlying challenges to the constrained optimization approach. For one, 
However, the fairness constraints are often irregular and have to be relaxed in order to optimize.
Notably, our method does not use the constraints directly in the model loss, and thus does not require them to be relaxed. %\cite{cotter2018optimization} has tried to address this issue, which leads to a complicated swap-regret strategy solving a non-zero-sum game.
Moreover, these approaches typically are not readily applicable to equality constraints as feasibility challenges can arise; thus, there is the added challenge of determining appropriate slack during training. Finally, the training can be difficult as \cite{cotter2018optimization} has shown that the Lagrangian may not even have a solution to converge to. 

When the classification loss and the relaxed constraints have the same form (e.g. a hinge loss as in~\cite{eban2017scalable}),
the resulting Lagrangian may be rewritten as a cost-sensitive classification, explicitly pointed out in \cite{agarwal2018reductions}, who show that the Lagrangian method reduces to solving an objective of the form $\sum_{i=1}^n w_i \1 [h(x_i) \neq y_i']$ for some non-negative weights $w_i$. In this setting, $y_i'$ may not necessarily be the true label, which may occur for example in demographic parity when the goal is to predict more positively within a protected group and thus may be penalized for predicting correctly on negative examples. %While this may be a reasonable approach to achieving fairness, it could be interpreted as training a weighted loss on {\it modified} labels, which may be legally prohibited \cite{barocas2016big}.
In contrast, our approach is a non-negative re-weighting of the original loss (i.e., does not modify the observed labels) and is thus simpler and more aligned with intuition. %legal standards. %Thus, in the context of fairness, our approach can be viewed as a simplified way to solve what the Lagrangian methods aims to achieve, but in a more direct fashion.

%OFIR COMMENTED In certain situations, the relaxed constraints can essentially be viewed as a linear combination of the losses for each datapoint. %For example, in the case of equal opportunity, a fairness constraint could be the difference between the true positive rate for a protected group and that of the entire dataset. %Thus, a relaxed constraint would be based on difference between the average loss on the positive examples of the protected group and the positive examples of the overall dataset. Thus, 
%OFIR COMMENTED In these cases, the Lagragianian would then be a reweighting of the original loss. Hence, our approach accomplishes what constrained optimization ideally tries to achieve in such situations, but perhaps in a more direct fashion. Moreover, our framework may provide further insights and implications to constrained optimization. % but in a more direct fashion, by guaranteeing fairness on the original constraints instead of the relaxed ones, while training based on the the relaxed ones, and avoiding many of the practical difficulties of training in such a manner in the constrained optimization setting, such as solving a non-zero-sum two-player game \cite{cotter2018two,cotter2018optimization}. %\footnote{To our knowledge, the only variant of constrained optimization which guarantees fairness on the original (and not relaxed) constraints is \cite{cotter2018two,cotter2018optimization}, but this methods requires solving for an approximate equilibrium to a non-zero-sum two-player game using a complex swap-regret method and cannot easily yield a deterministic classifier in practice. Interestingly, the assumptions of our framework allows our method to solve the constrained optimization in a more direct way, without having to find an equilibrium to a two-player game as an intermediate step while having theoretical guarantees.}

{\bf Pre-processing:} This approach has primarily involved massaging the data to remove bias. Examples include \cite{calders2009building,kamiran2009classifying,vzliobaite2011handling,kamiran2012data,zemel2013learning,fish2015fair,feldman2015certifying,beutel2017data}. Many of these approaches involve changing the labels and features of the training set, which may have legal implications since it is a form of training on falsified data \cite{barocas2016big}. Moreover, these approaches typically do not perform as well as the state-of-art and have thus far come with few theoretical guarantees \cite{krasanakis2018adaptive}.
In contrast, our approach does not modify the training data and only re-weights the importance of certain sensitive groups. Our approach is also notably based on a mathematically grounded formulation of how the bias arises in the data. 

